MMGA: Multimodal Learning with Graph Alignment

Multimodal pre-training breaks down the modality barriers and allows the individual modalities to be mutually augmented with information, resulting in significant advances in representation learning. However, graph modality, as a very general and important form of data, cannot be easily interacted with other modalities because of its non-regular nature. In this paper, we propose MMGA (Multimodal learning with Graph Alignment), a novel multimodal pre-training framework to incorporate information from graph (social network), image and text modalities on social media to enhance user representation learning. In MMGA, a multi-step graph alignment mechanism is proposed to add the self-supervision from graph modality to optimize the image and text encoders, while using the information from the image and text modalities to guide the graph encoder learning. We conduct experiments on the dataset crawled from Instagram. The experimental results show that MMGA works well on the dataset and improves the fans prediction task's performance. We release our dataset, the first social media multimodal dataset with graph, of 60,000 users labeled with specific topics based on 2 million posts to facilitate future research.

==> experiment.tex <==
 %!TEX root  = pretrain.tex
\section{Experiments}

\subsection{Experimental setting}



\begin{table}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Dataset&items&Rising stars&users&Taocode\\
		\hline
		CLOTH&10000&3210&7.9M&6.1M\\
		\hline
		FOOD&10000&1895&14.2M&17.0M\\
		\hline
		COSMETIC&10000&1777&13.6M&13.4M\\
		\hline
		NECESSITIES&10000&1465&14.5M&15.7M\\
		\hline
		
	\end{tabular}
	\caption{Datasets overview}
	\label{tab:dataset}
\end{table}

\subsection{Baseline Methods}
We compare our proposed model with the following baselines and the details of these baselines are in the appendix:
\begin{itemize}[leftmargin=*] 
    \item \textbf{MMGCN~\cite{wei2019mmgcn}}. MMGCN is a graph-based algorithm. To learn representations of user preferences on different modalities, it devises a model-specific bipartite graph based on the user-item interactions for each modality. After that, it aggregates all model-specific representations to obtain the representations of users or items for prediction.
    \item \textbf{PMGT~\cite{liu2021pre}}. Pre-trained Multimodal Graph Transformer, which exploits items’ multimodal information guided by the unsupervised learning tasks on graph.
    \yx{check}
    \item \textbf{new baseline}. TransAE [37]: This method combines a multimodal
    encoder and the TransE [2] model to learn the node representations; 6) GRAPH-BERT [39]: This method applies Transformer to aggregate neighbors’ information without masking operations on the nodes; 7) GPT-GNN [15]: This method employs the attribute generation and edge generation tasks to pre-train the GNN model.
    For a fair comparison, we use the same multimodal representation in Eq. (3) as the inputs for all pre-training methods.
    \item \textbf{GRCN}.
    \item \textbf{DualGNN}.
    \item \textbf{LATTICE}.
\end{itemize}

\subsection{Performance Comparison}
\vpara{Pretrain task} 

\subsection{Ablation Study}
To validate the contribution of each component of our proposed model GFR, we conduct ablate study on four different analytical aspects listing below:
\begin{itemize}[leftmargin=*] 
	\item \textbf{Effect of pretrain task one} MMGA-g:
\end{itemize}

\subsection{Case Study}



==> observation.tex <==
%!TEX root = pretrain.tex

\section{DATA COLLECTION AND ANNOTATION}
\subsection{Dataset Collection}
\subsection{Dataset labeling}
\subsection{Graph construction}
\label{sec:observation}



==> preliminary.tex <==
%!TEX root = pretrain.tex
\section{Preliminaries}
\label{sec:data}


==> related.tex <==
%!TEX root = pretrain.tex
\section{Related Work}
In the interests of clarity, we first review multimodal methods, then introduce graph related works. 
\subsection{Multimodal learning}
There have been many attempts to unify various vision and language tasks into a single framework.
\subsection{Multi-modal personalized recommendation}
Personalized recommendation systems have been successfully applied to many applications, such as e-commerce, news, and social media platforms. In particular, some efforts have been dedicated to integrate the item features, which are extracted from multiple modalities by the pre-trained deep learning models, into the CF based model for enhancing the item representations.

